Lobbying Influence -- The Role of Money, Strategies and Measurements

Comparing the results for preference attainment, self-perceived influence and reputational influence, this paper analyzes the relationship between financial resources and lobbying influence. The empirical analysis builds on data from an original survey with 312 Swiss energy policy stakeholders combined with document data from multiple policy consultation submission processes. The results show that the distribution of influence varies substantially depending on the measure. While financial resources for political purposes predict influence across all measures, the relationship is positive only for some. An analysis of indirect effects sheds light on the potential mechanisms that translate financial resources into influence.

==> files_mediation.draft/table_template.tex <==
\centering
\caption{Descriptive statistics} 
\label{tab:descriptive}
\begingroup\fontsize{9pt}{10pt}\selectfont
\begin{tabular}{lrrr}
  \hline
\addlinespace
  & Mean & Median & SD \\
\addlinespace
 \hline
  \addlinespace
\multicolumn{4}{l}{\textbf{\textit{Data 1}}} \\
\addlinespace
Variable 1 & 0.50 & 0.46 & 0.29 \\ 
  Variable 2 & 0.22 & 0.00 & 0.42 \\ 
   \addlinespace
\multicolumn{4}{l}{\textit{Variable 3}} \\
\quad Low & 0.06 & 0.00 & 0.24 \\ 
  \quad Medium & 0.47 & 0.00 & 0.50 \\ 
  \quad High & 0.26 & 0.00 & 0.44 \\ 
  \quad Very high & 0.21 & 0.00 & 0.41 \\ 
   \addlinespace
Variable 4 & 998.16 & 987.35 & 102.14 \\ 
   \addlinespace
\multicolumn{4}{l}{\textbf{\textit{Data 2}}} \\
\addlinespace
Variable 1 & 4.04 & 4.05 & 0.56 \\ 
  Variable 2 & 0.49 & 0.00 & 0.50 \\ 
   \addlinespace
\multicolumn{4}{l}{\textit{Variable 3}} \\
\quad Very low & 0.06 & 0.00 & 0.23 \\ 
  \quad Low & 0.10 & 0.00 & 0.29 \\ 
  \quad Medium & 0.38 & 0.00 & 0.49 \\ 
  \quad High & 0.31 & 0.00 & 0.46 \\ 
  \quad Very high & 0.16 & 0.00 & 0.37 \\ 
   \addlinespace
Variable 4 & 2007.38 & 2013.32 & 317.44 \\ 
   \addlinespace
\hline
\addlinespace
\end{tabular}
\endgroup

